Combating Uncertainties in Wind and Distributed PV Energy Sources Using Integrated Reinforcement Learning and Time-Series Forecasting

Renewable energy sources, such as wind and solar power, are increasingly being integrated into smart grid systems. However, when compared to traditional energy resources, the unpredictability of renewable energy generation poses significant challenges for both electricity providers and utility companies. Furthermore, the large-scale integration of distributed energy resources (such as PV systems) creates new challenges for energy management in microgrids. To tackle these issues, we propose a novel framework with two objectives: (i) combating uncertainty of renewable energy in smart grid by leveraging time-series forecasting with Long-Short Term Memory (LSTM) solutions, and (ii) establishing distributed and dynamic decision-making framework with multi-agent reinforcement learning using Deep Deterministic Policy Gradient (DDPG) algorithm. The proposed framework considers both objectives concurrently to fully integrate them, while considering both wholesale and retail markets, thereby enabling efficient energy management in the presence of uncertain and distributed renewable energy sources. Through extensive numerical simulations, we demonstrate that the proposed solution significantly improves the profit of load serving entities (LSE) by providing a more accurate wind generation forecast. Furthermore, our results demonstrate that households with PV and battery installations can increase their profits by using intelligent battery charge/discharge actions determined by the DDPG agents.

==> Chapters/Formulation_old.tex <==
\section{System Model and Problem Formulation}

\subsection{Power Market Model}

\begin{figure}
\centering
    \includegraphics[scale=0.28, trim =1.5cm 3.1cm 0.5cm 0.1cm, clip]{LSTM+DQN/Figures/Model.png}
    \caption{Electricity market structure with presence of prosumer and wind power plant
    }
    \label{Model}
    \vspace{-.15in}
\end{figure}
As a result of integrating wind power production uncertainty into the energy market, this study is aimed to develop a decision-making framework that combat the wind generation uncertainties, while  optimizing the economic benefits for services provider and residential users. To this end, Figure.\ref{Model} illustrates the system model, which includes active prosumers that are equipped with PV panels and energy storage system units. Furthermore, the load serving entity (LSE) is responsible for aggregating load on behalf of many residential users and making appropriate arrangements in wholesale markets to meet that load.
Independent System Operators (ISOs) and Regional Transmission Organizations (RTOs) are responsible for keeping the power grid balanced between generation and load.
Wind power production as renewable generation as well as conventional power plants are considered as different type of generation.

Our envisioned energy market consists of both day-ahead (DA) and real-time (RT) markets. The ISO/RTO receives the generation and demand from the market participants and determines the clearing price and clearing power quantities of the market. The wind power plant is assumed to be a price-taker and trade power in real-time and day-ahead markets. Additionally, conventional power plants (CPP) participate by submitting their price and power output to the ISO, which determines the locational marginal price (LMP).  After the LMPs are determined, the LSE sets the electricity buy and sell price with considering status of the prosumers.
Status of prosumers are determined to be selling or buying energy from the LSE, depending on their PV generation, energy consumption, and battery state of charge. 
% buy energy from the declares the amount of energy they will purchase or sell from the LSE.

% DSO collects all data on power quantities and prices from market participants, and based on network constraints, determine the clearing price and clearing power quantities of the market.
% In order to include the uncertainty of wind power production in day-ahead energy forecasting, wind generation is considered as a type of generation, and its power output is predicted using a forecasting engine. Actual values of wind power generation have been compared with the predictions from the forecasting engine. As a result, the level of wind power penetration uncertainty has been investigated by measuring the prediction error. 

According to Figure \ref{Model}, we have a two-level optimization problem. The LSE collects wholesale market prices and power quantities from wholesalers at the upper-level while considering the prosumer status. The LSE dynamically determines the electricity buy and sell price based on the collected data.
% Figure \ref{supply} shows the price and cost curve for each power producer. According to the figure, failure to predict the actual results to an extra cost for the DSO, which is illustrates as the red shaded region. As a result, DSO needs to capture the wind generation uncertainty with a forecasting tool.
Additionally, prosumers receive electricity prices and decide whether to charge or discharge their batteries on the lower-level. As a result, an upper-level optimization problem consists of determining the price of electricity by LSE to improve its profit, while a lower-level problem involves active prosumer taking action on their batteries in an attempt to reduce their electricity bills.




\subsection{Residential-users}
Residential users include active prosumers ($\mathcal{N^P}$) who own PV solar panels and energy storage systems (ESS), as well as passive consumers ($\mathcal{N^C}$). Therefore, each residential side user $i$ will be either an active prosumer or a passive consumer as follows, $ i \in \mathcal{D} = \left\{ \mathcal{N^P} \cup \mathcal{N^C} \right \}$. The active prosumers' energy trading amount at time slot $t$ is defined as follows:
\begin{equation}\label{eq:pro}
e_{i,t} = d_{i,t}-g_{i,t}-b_{i,t},\:\: \forall i \in \mathcal{N^P},
\end{equation}
where $d_{i,t}$, $g_{i,t}$, and $b_{i,t}$ denote the energy consumption, PV generation, energy charge/discharge from the battery, respectively. 
% According to \eqref{eq:CostLSE}, if the $e_i(t)$ is non-negative $\lambda_i = 0$, which means the prosumer $i$ is need to buy the energy from the LSE. Otherwise, $\lambda_i = 1$ which means the prosumer sell its excess energy back to LSE.
In addition, the $L_{i,t}$ for each prosumer and consumer is defined in \eqref{eq:demand} that determines the load, i.e.,: 
\begin{equation}\label{eq:demand}
    {L_{i,t}}=\begin{cases}
        d_{i,t} & \text{if} \; i \in \mathcal{N^C}\\
    e_{i,t} & \text{if} \; i \in \mathcal{N^P}. 
            \end{cases}
\end{equation}
Therefore, the aggregated load that represents the energy transfer between the LSE and residential users is obtained as follows:
\begin{equation}\label{eq:Aggload}
L^D_t =  \sum\limits_{i=1}^{{\mathcal{D}}}{L_{i,t}}.
\end{equation}


The revenue of each prosumer is calculated based on its excess energy generation by the PV setup as well as its  energy demand. According to \eqref{eq:prosumerobj}, if the $e_{i,t}$ is non-negative $\lambda_i = 0$, which means the prosumer $i$ needs to buy the energy from the LSE. Otherwise, $\lambda_i = 1$ which means the prosumer sells its excess energy back to the LSE. The prosumer's electricity bill is calculated as follows:
% (or we can mention considering the electricity bills of prosumer and consumers and try to minimize the aggregated load)
\begin{equation}\label{eq:prosumerobj}
\mathcal{E}_i^{pro} = \sum_{t \in T} \left \{ (1-\lambda_i) e_{i,t}C^s_t + \lambda_i e_{i,t}C^b_t \right \} ,\:\: \forall i \in \mathcal{N^P}.
\end{equation}

\textbf{Energy Storage System:} The prosumer batteries are modeled by the general ESS characterization such as, charging and discharging rate, maximum capacity, state of charge of the battery, and the battery efficiencies, as follows:
\begin{equation}\label{eq:batttery_limit}
 SoC^{{\min}}_{i} \le \frac{1}{{{Q_i}}}\sum_{t\in\ T}{b_{i,t}} + So{C_{{i}}}(0) \le SoC^{{\max}}_{i},\: \forall i \in \mathcal{N^P,} 
\end{equation}



\begin{equation}\label{eq:battery charge\discharge}
  b^{dis,min}_{i} \le b_{i,t}\le b^{charge,max}_{i},\: \forall i \in \mathcal{N^P}.
\end{equation}


\textbf{PV Generation:} Solar PV panels are considered as a distributed energy resource for active prosumers. The prosumers will produce energy to meet their demand, charge their battery, or sell the energy back to the grid during the peak generation times or high price periods. There is a non-negative constraint for PV generation, but it must be limited by their maximum generation capacity, which is shown as follows:
\begin{equation}\label{eq:PV constraint}
  0\le\ g_{i,t} \le g^{\text{max}}_{i},\: \forall i \in \mathcal{N^P}.
\end{equation}




\subsection{Load Serving Entity}
% \textbf{Distribution System Operator:}  DSO in the upper-level model seeks to minimize the total cost of the system or maximize their own total payoff, while incorporating the uncertainty in wind power production. To this end, the wind power production will be determined by a LSTM forecasting engine. The total cost (TC) that needs to be minimized by DSO is defined as follows:

LSE in the upper-level model seeks to minimize the total cost or maximize its own total payoff, while incorporating the uncertainty in wind power production and demand uncertainty. To this end, an LSTM forecasting engine is used to determine the wind power production that is directly related to the LMP. The total cost (TC) of the LSE is defined as follows:
\begin{align}
    \begin{aligned}
        TC = \sum_{t\in\ T} \left\{ {L^{DA}_t {\rho}^{DA}_t} +\sum\limits_{i = 1}^{\mathcal{N^P}} |e_{i,t}|C^b_t\lambda_i + \Delta L_t {\rho}^{RT}_t \right\}.\label{eq:CostLSE}
    \end{aligned}
\end{align}

The TC incorporates the total cost of the LSE to procure energy from the wholesale market as well as from the distributed energy sources, i.e., active prosumers.
The first term in \eqref{eq:CostLSE} indicates that the LSE purchases $L^{DA}$ at $\rho^{DA}$ in the DA market. Furthermore, the LSE purchases $e_i$ from the $i^{th}$ active prosumer with the electricity buy price determined by the LSE. In this equation, $\lambda_i$ shows the prosumers that tend to help the LSE where $\lambda_i = 1$ represents the prosumer that is supporting the LSE by selling energy back to it.  $\Delta L_t =  L^{RT}_t - L^{DA}_t$ is the DA and RT demand deficiency to calculate the LSE cost for the load uncertainty in the RT market.
As a result, the LSE net profit can be calculated by subtracting the LSE costs from the aggregated residential energy demand. 
\begin{align}
    \begin{aligned}
        \mathcal{R}^{LSE} = \sum_{t\in\ T} \left\{ \sum\limits_{j=1}^{\mathcal{N^C}}{L_{j,t}^{RT}C_t^s} + \sum\limits_{k=1}^{\mathcal{N^P}}{L_{k,t}^{RT}C^{s}_t} \right\} - TC. \label{eq:RevLSE}
    \end{aligned}
\end{align}

% The next step is to define the components for both residential users and energy providers in the proposed system.


% \begin{align}
%     &\min_{C_b, C_s}
%     \begin{aligned}
%         TC = \sum_{t\in\ T} \left\{ {P^{WP}(t)C^{WP} + \sum\limits_{n=1}^{N_g}P_n^G(t)C_n^G} \\+\sum\limits_{k = 1}^{N_p} P_{k}^{pro}(t)C_b(t) - P^D(t)C_s(t) \right\}\label{eq:DSO}
%     \end{aligned} \\
%     &\text{Subject to:} \notag\\
%     &{P^{WP}(t) + P^G(t) + \sum\limits_{k = 1}^{N_p} P_k^{pro} (t) - P^D(t) = 0}, \label{eq:balance1}\\
%     & P^D(t) = P^{con} + P^{pro}\label{eq:demand} \\
%     & P^G(t) = \sum\limits_{n =1}^{N_g}P_{n}^G(t) + P^{WP}(t),\label{eq:Gen} \\
%     & P_n^{G,\min} \le P_{n}^G(t) \le P_n^{G,\max},\label{eq:GenLimits} \\
%     & 0 \le P^{WP}(t) \le P^{WP,\max} \label{eq:WindLimit},
% \end{align}


% The power balance equation is provided in \eqref{eq:balance1}, \eqref{eq:demand} and \eqref{eq:Gen} indicate amount of demand and generation respectively, \eqref{eq:GenLimits} shows conventional generation limits, and the wind power generation limit is shown in \eqref{eq:WindLimit}. As we discussed earlier, the first term in equation \eqref{eq:DSO} refers to purchased power from wind generation. Due to the volatile nature of wind power generation, the amount of wind energy is calculated with a forecasting engine. So, the DSO optimization problem can be rewritten as  following:

% \begin{align}
%     &\min_{C_b, C_s}
%     \begin{aligned}
%         TC = \sum_{t\in\ T} \left\{ {\Delta P^{WP}(t)C^{RT}(t) + \sum\limits_{n=1}^{N_g}P_n^G(t)C_n^G} +\\ \sum\limits_{k = 1}^{N_p} P_{k}^{pro}(t)C_b(t) - P^D(t)C_s(t) \right \}\label{eq:DSO2}
%     \end{aligned} \\
%     & \Delta P^{WP}(t) = |P^{WP}_{actual}(t) - P^{WP}_{preds}(t)|.\label{eq:windP}
% \end{align}

% The optimization problem in \eqref{eq:DSO2} is the new problem with incorporating the wind power generation uncertainties. Also, \eqref{eq:windP} calculates the difference between wind power actual and forecasted values. 





% \subsection{Energy Storage and Generation Model}
% \textbf{Energy Storage System:} The prosumer batteries are modeled by the general ESS characterization such as, charging and discharging rate, maximum capacity, state of charge of the battery, and the battery efficiencies, as follows:
% \begin{equation}\label{eq:batttery_limit}
%  SoC^{{\min}}_{i} \le \frac{1}{{{Q_i}}}\sum_{t\in\ T}{b_{i,t}} + So{C_{{i}}}(0) \le SoC^{{\max}}_{i},\: \forall i \in \mathcal{N^P,} 
% \end{equation}



% \begin{equation}\label{eq:battery charge\discharge}
%   b^{dis,min}_{i} \le b_{i,t}\le b^{charge,max}_{i},\: \forall i \in \mathcal{N^P}.
% \end{equation}


% \textbf{Power Generation:} Solar PV panels are considered as a distributed energy resource for active prosumers. The prosumers will produce energy to meet their demand, charge their battery, or sell the energy back to the grid during the peak generation times or high price periods. There is a non-negative constraint for PV generation, but it must be limited by their maximum generation capacity, which is shown as follows:
% \begin{equation}\label{eq:PV constraint}
%   0\le\ g_{i,t} \le g^{\text{max}}_{i},\: \forall i \in \mathcal{N^P}.
% \end{equation}

% According to Figure~\ref{Model}, conventional power plants are considered as one type of generator, along with wind power plant as a type of renewable energy sources. 
% % A wind power plant is considered for assessing the uncertainty caused by intermittent wind generation.
% Each generation facility $i \in \mathcal{N_G}$ has a minimum and maximum generation limit, as described in \eqref{eq:GenLimits} and \eqref{eq:Wind constraint}. The generation ramp rate is defined in \eqref{eq:GenRamp} to demonstrate how quickly a plant can change its output.
% \begin{equation}\label{eq:GenLimits}
%   P_i^{G,\min} \le P_{i,t}^G \le P_i^{G,\max}, \forall i \in \mathcal{N^G},
% \end{equation}
% \begin{equation}\label{eq:Wind constraint}
%   0\le\ P_t^{wp} \le P^{wp,\text{max}},
% \end{equation}
% \begin{equation}\label{eq:GenRamp}
%   RR_i^{\min} \le P_{i,t+1}^G - P_{i,t}^G \le RR_i^{\max}, \forall i \in \mathcal{N^G}.
% \end{equation}


\subsection{Power Balance and Energy Costs}
The ISO/RTO is responsible for maintaining the balance between demand and generation, as shown in Figure. \ref{Model}. The ISO collects the demand and generations from the LSE and power producers, respectively. Accordingly, the system marginal price and the generators' power commitment will be determined for the whole system.
To calculate the LMP, the formulation in \cite{fang2016strategic} is utilized by the ISO to determine the system LMP price while maintaining the system constraints. For both DA and RT markets, LMPs are calculated. Power balance is a major factor in determining LMP, and LMP is determined based on the cost of a generator that could clear the market.
% The impact of wind power uncertainty on the LMP price is also taken into account.
Therefore, power balance equation is defined as follows:
\begin{equation}\label{eq:Powerbalance}
  \sum\limits_{i = 1}^{\mathcal{D}} L_{i,t}   = \sum\limits_{i=1}^{\mathcal{N^G}} P_{i,t}^{G} + P^{wp}_t,
\end{equation}
where the aggregated demand of the residential users in the left-hand side should be met by the power producers, as well as wind power generator that is indicated as $P^{wp}(t)$.


According to Figure~\ref{Model}, conventional power plants are considered as one type of generator, along with wind power plant as a type of renewable energy sources. 
% A wind power plant is considered for assessing the uncertainty caused by intermittent wind generation.
Each generation facility $i \in \mathcal{N_G}$ has a minimum and maximum generation limit, as described in \eqref{eq:GenLimits} and \eqref{eq:Wind constraint}. The generation ramp rate is defined in \eqref{eq:GenRamp} to demonstrate how quickly a plant can change its output.
\begin{equation}\label{eq:GenLimits}
  P_i^{G,\min} \le P_{i,t}^G \le P_i^{G,\max}, \forall i \in \mathcal{N^G},
\end{equation}
\begin{equation}\label{eq:Wind constraint}
  0\le\ P_t^{wp} \le P^{wp,\text{max}},
\end{equation}
\begin{equation}\label{eq:GenRamp}
  RR_i^{\min} \le P_{i,t+1}^G - P_{i,t}^G \le RR_i^{\max}, \forall i \in \mathcal{N^G}.
\end{equation}



% %%%%%%%%  LMP price formulation %%%%%%%%%%%%%%%%%%
% \begin{align}
%     &\forall \rho \in arg
%     \begin{aligned}
%         &\left\{ \textbf{min} \sum_{t\in\ T} (\sum \limits_{i = 1}^{\mathcal{N_G}} P_{i}^{G}(t)C_i(t))+P^{wp}(t)C_{wp}(t) \right \} \label{eq:LMP}
%     \end{aligned}\\
%     &\text{Subject to:}\; \eqref{eq:GenLimits}\; \text{\&} \; \eqref{eq:GenRamp} \notag\\
%     & \sum \limits_{i = 1}^{\mathcal{D}} L_i(t)   = \sum \limit_{i=1}^{\mathcal{N_G}} P_{i}^{G}(t) + P^{wp}(t)\label{eq:Powerbalance}
% \end{align}





\subsection{Wind Power Uncertainty}
As mentioned earlier,  wind power is an important renewable energy source. However, in contrast to the conventional power generation sources, the output of a wind farm is uncertain. As shown in Figure~\ref{Model}, our system model considers the wind power  in the generator side. The intermittent and uncertain output of wind generation, however, could result in mismatch between the power production and electricity demand. Additionally, the wind power uncertainty will affect the LMP price. Therefore, failing in estimating the wind power results in high cost for the system participants. For instance, if the LSE is unable to predict wind power accurately, then it must purchase power on the spot market or purchase from costly spinning reserve generators.

Figure~\ref{supply} provides the supply and demand curve in the presence of various power producers. The effect of having accurate wind power estimation is illustrated in this figure, where the red curve demonstrates the power generation with having wind power forecasting and the blue curve is with actual wind power. The failure to estimate wind power accurately, even when load demand is lower, will result in a higher LMP. As a result, there would be a significant increase in the cost of the system because of this mismatch between the predicted wind generation vs. the actual generation.
% The long-short term memory was utilized as a forecasting engine in order to solve the problem of inaccurate forecasting.

% Next, we present the optimization problems for the residential users and LSE.

\begin{figure}[h]
  \centering
    \includegraphics[scale=0.45, trim = 0.1cm 0.2cm 0.2cm 0.2cm, clip]{LSTM+DQN/Figures/supply.png}
    \caption{Generator prices and supply cost curve}
    \label{supply}
    % \vspace{-.2in}
\end{figure}



\









\subsection{Optimization Problem}
According to the problem setup so far, we have a two-level optimization problem. On one hand, in the residential user level, active prosumers aim to reduce their electricity bills. On the other hand, the LSE primary goal is to maximize its profit. Given these two observations, the optimization problems can be defined as follows.

\textbf{Residential user level:} In the residential user level market, the participant ultimate goal is to reduce  electricity bills. To this end, prosumers decide to take an action on their batteries after receiving the electricity price from the LSE. In this regard, the optimization problem in the residential level can be defined as follows:
% \begin{align}
%     &\min_{b_i}
%     \begin{aligned}
%         EB = \sum_{i\in\ \mathcal{N^P}}\mathcal{R}_i^{pro}  \label{eq:UserLevel}
%     \end{aligned}\\
%     &\text{Subject to:} \eqref{eq:pro} \textbf{\&} \eqref{eq:demand} \textbf{\&} \eqref{eq:batttery_limit} \textbf{\&} \eqref{eq:battery charge\discharge} \notag
% \end{align}
\begin{equation}
 \textbf{User level:} 
 \begin{cases}
 \mathop{\mathrm{minimize}}\limits_{b_i} & \sum\limits_{i\in\mathcal{N^P}}\mathcal{E}_i^{pro},   \\ 
\text{subject to:} & \eqref{eq:pro} \textbf{\&} \eqref{eq:demand} \textbf{\&} \eqref{eq:batttery_limit} \textbf{\&} \eqref{eq:battery charge\discharge}.  
\label{eq:UserLevel}
\end{cases}
\end{equation}


% \textbf{Distribution-level:} In the distribution-level market, the participant ultimate goal is to reduce their electricity bills. Prosumers decide to act on their battery after learning the electricity price from the DSO. 
% % In order to include the consumer in the market model, the concept of consumer benefit must be introduced. Consumer benefit represents the value the consumer gains from using a product.
% Thus, the lower-level problem is formulated as follows:

% \begin{align}
%     &\min_{P^B_k}
%     \begin{aligned}
%         & EB = \sum_{t\in\ T} \left\{ P_{k}^{pro+}(t)C_s-P_{k}^{pro-}(t)C_b \right \} \label{eq:prosumer}
%     \end{aligned}\\
%     &\text{Subject to:} \notag\\
%     &P_{k}^{pro}(t)= P_{k}^{PV}(t) - P_{k}^B(t) - P^C_{k}(t)\label{eq:Powerbalance}\\
%     & SoC^{{B, \min}}_{k } \le \frac{1}{{{Q^{B}_k}}}\sum_{t\in\ T}{{P^{B}_{k}}(t)} + So{C_{{b_j}}}(0) \le SoC^{{B, \max}}_{k } \label{eq:batttery_limit}, \\
%   & P^{B,min}_{k} \le P^{B}_{k}(t)\le P^{B,max}_{k} \label{eq:battery charge\discharge constraint}, \\
%   & 0\le\ P^{PV}_{k}(t) \le P^{PV,\text{max}}_{k}\label{eq:PVconstraint},
% \end{align}

The objective function \eqref{eq:UserLevel} takes into account the cost of purchasing energy from the LSE and subtracts the quantity of energy sold back.
This optimization problem is subjected to prosumers' power balance equation, battery charging and discharging limits, as well as PV panel generation limit. The control variable in this optimization problem will be charging or discharging the prosumers' battery.

% The power balance equation is provided in \eqref{eq:Powerbalance}, also state of charge of the battery, battery charging and discharging limits, and PV panel generation limit are provided in \eqref{eq:batttery_limit} to \eqref{eq:PVconstraint}, respectively. According to \eqref{eq:Powerbalance}, $&P_{k}^{pro}$ can take positive or negative values depending on the amount of PV generation and battery charge or discharge action.
% % Equivalent optimization problem with difference of forecasting and actual


\textbf{LSE-level:} In the upper-level market, LSE aims to maximize its own profit. LSE is trying to achieve this objective through changing the electricity buy and sell price. Therefore, the optimization problem in the LSE-level can be defined as follows:
% \begin{align}
%     &\max_{C^b, C^s}
%     \begin{aligned}
%         \mathcal{R}^{LSE} \label{eq:LSEobj}
%     \end{aligned} \\
%     &\text{Subject to:} \notag\\
%     &\eqref{eq:GenLimits} \textbf{\&} \eqref{eq:Wind constraint} \textbf{\&} \eqref{eq:GenRamp} \textbf{\&} \eqref{eq:Powerbalance} \notag
% \end{align}
\begin{equation}
 \textbf{LSE level:} 
 \begin{cases}
 \mathop{\mathrm{maximize}}\limits_{C^b, C^s} & \mathcal{R}^{LSE},   \\ 
\text{subject to:} & \eqref{eq:GenLimits} \textbf{\&} \eqref{eq:Wind constraint} \textbf{\&} \eqref{eq:GenRamp} \textbf{\&} \eqref{eq:Powerbalance}.  
\label{eq:LSEobj}
\end{cases}
\end{equation}
The objective function in Eq. \eqref{eq:LSEobj} incorporates power procurement from the wholesale energy market, also the amount of energy selling to the residential-users. This objective is subject to power generation limits, generation ramp rate limit, and also the power balance equation, as described earlier. 






















==> Chapters/LSTM.tex <==
\section{Wind power forecast model}
\hl{Some brief intro about forecasting methods for wind can be mentioned here}
\subsection{Convolutional and Recurrent Neural Network}

A convolutional neural network (CNN) is a multi-layer feed-forward artificial neural network that has a convolutional layer, a pooling layer, and a fully connected layer.
The convolutional layer use a filter to create a feature map from input data and pass it to the pooling layer. Pooling layer is responsible to reduce data dimension by combining the output of neurons. The fully connected layer is the final layer of CNN and do the classification of the input data. CNN has the ability to capture the spatial features of input data, but it is incapable of effectively interpreting the temporal information. Thus, it is highly effective in image recognition and classification tasks. 
Recurrent neural network (RNN) is another type of artificial neural network which uses sequential data or time series data. Unlike the traditional neural network, in RNN the output from previous step are fed as input to the current step, which is called hidden state. Hidden state is used to remember some information about a sequence. This RNN feature make it a perfect choice for prediction problems, such as speech recognition, and natural language processing. Although, the RNN has a vanishing gradient, and also the long-term dependency problem. One way to avoid these problems is using LSTM method.



\subsection{Long short term memory (LSTM)}

LSTM is an enhanced version of RNN. The original idea of LSTM is proposed by \cite{101162} to overcome RNN shortcoming.
% the RNN vanishing gradient problem and also to avoid the long-term dependency problem.
Also, various optimized LSTM model has been proposed to enhance the LSTM performance, such as \cite{GRAVES2005602,861302}. The LSTM has been applied to various type of problems such as, speech recognition \cite{6707742}, image captioning \cite{ZHU201855},  language translation \cite{wu2016google}, and time-series forecasting \cite{KAREVAN20201}. Fig. \ref{LSTM} shows the structure of LSTM. A LSTM unit is composed of a cell, and within the cell, three gates control the flow of information within the LSTM cell and control the cell state. The three gates are: an input gate, an output gate, and a forget gate.
The three gates, forget, input, and output, can be seen in the Fig. \ref{LSTM} as $f_t$, $i_t$, and $o_t$, respectively.
\begin{figure}[h]
   \centering
    \includegraphics[scale=0.32, trim = 0.5cm 0.5cm 0.5cm 0.5cm, clip]{Figures/StackLSTM.png}
    \caption{Stacked LSTM model and a LSTM cell architecture}
    \label{LSTM}
    % \vspace{-.2in}
\end{figure}


The forget gate tells the cell which information to throw away from the internal cell state via activation function. Also, the input gate tells the cell which new information to store in the internal cell state. Output gate will decide whether to pass the information to the next neuron or not. LSTM unit function are mathematically formulated as follows:
\begin{equation}\label{eq:forget}
    f_t = \sigma (W_f \cdot <h_{t-1},X_t> + b_f),
\end{equation}

\begin{equation}\label{eq:input}
    i_t = \sigma (W_i \cdot <h_{t-1},X_t> + b_i),
\end{equation}

\begin{equation}\label{eq:output}
    o_t = \sigma (W_o \cdot <h_{t-1},X_t> + b_o),
\end{equation}

\begin{equation}\label{eq:cell}
    \begin{aligned}
        \hat{C_t} & = tanh (W_c \cdot <h_{t-1},X_t> + b_c), \\
        &\C_t = i_t \cdot \hat{C_t} + f_t \cdot C_{t-1},   
    \end{aligned}
\end{equation}

\begin{equation}\label{eq:hidden}
    h_t = o_t \times tanh(C_t),
\end{equation}

where $f_t$, $i_t$, and $o_t$ represent the forget gate, input gate, and output gate at time step $t$, respectively. $\hat{C_t}$ represents a temporary state and $C_t$ is the state of the LSTM at time step t. $W$ is the weight matrix for each gate, and $b$ is the bias. $\sigma$ and $tanh$ are the sigmoid and tanh activation function. $X_t$ is the input, and $h_t$ is the output at time step $t$.

The LSTM network with more than one hidden layer is called stacked or deep LSTM. Stacked LSTM consists of multiple layers of LSTM, with the output of the previous layer becoming the input to the next layer. The architecture of a stacked LSTM is illustrated in Fig.\ref{Stack}. Stacked LSTM cells can store more information through hidden layers. Each LSTM layer processes some portion of the task and transfers the output to the next layer. Finally, the results are taken from the output layer. Stacking of hidden layers makes the recurrent model deeper and can learn features more accurately. The concept of stacked or deep LSTM was first proposed by \cite{6638947}. Stacked LSTM is found to be a powerful technique for sequence prediction problems.

% \begin{figure}[h]
%   \centering
%     \includegraphics[scale=0.3, trim = 2cm 4cm 2cm 2cm, clip]{LSTM/Figures/StackedLSTM.png}
%     \caption{Stacked LSTM network}
%     \label{Stack}
%     % \vspace{-.2in}
% \end{figure}

\subsection{Gated Recurrent Network (GRU)}
GRU is another popular variant of RNN and simpler version of LSTM. GRU was introduced in 2014 \cite{cho2014learning}, which uses less training parameter and therefore uses less memory and executes faster than LSTM, whereas LSTM is more accurate on a larger dataset.To solve the vanishing gradient problem of RNN, GRU uses update gate and reset gate. 
The update gate is responsible for determining the amount of previous information that needs to pass along to the next state. This is really powerful because the model can decide to copy all the information from the past and eliminate the risk of vanishing gradient. The reset gate is used from the model to decide how much of the past information is needed to neglect; in short, it decides whether the previous cell state is important or not.      
% To explain the mathematics behind GRU process, we will examine a single unit is shown in Fig. \ref{GRU}.


% \begin{figure}[h]
%   \centering
%     \includegraphics[scale=0.4, trim = 0.2cm 0.1cm 0.2cm 0.2cm, clip]{LSTM/Figures/GRU.png}
%     \caption{GRU cell architecture}
%     \label{GRU}
%     % \vspace{-.2in}
% \end{figure}

The update gate formula for time step $t$ is:
\begin{equation}\label{eq:update}
    z_t = \sigma (W_z x_t + U_z h_{t-1}),
\end{equation}
where the input $x_t$ is multiplied by its own weight $W_z$, and $h_{t-1}$ the output from the previous time step is also multiplied by its own weight $U_z$. Both are added together and pass to a sigmoid activation function.The update gate helps the model to determine how much of the past information (from previous time steps) needs to be passed along to the future.
The reset gate is used to decide how much of the past information to forget.
\begin{equation}\label{eq:reset}
    r_t = \sigma (W_r x_t + U_r h_{t-1}),
\end{equation}
which is the same as the update gate, but the weight matrices $W_r$ and $U_r$ are different. $\widetilde{h_t}$ is a new memory content which uses the reset gate, the input, and the output from previous time step to store the relevant information from the past:
\begin{equation}\label{eq:tildeh}
    \widetilde{h_t} = tanh (W x_t + r_t \cdot U h_{t-1}).
\end{equation}
In the last step, the $h_t$ which is the information of the current unit should be calculated, and using the update gate $z_t$ will decide to keep the majority of information from the past ($z_t$ is close to 1) or keep more portion of the current content ($z_t$ is close to 0):
\begin{equation}\label{eq:outputGRU}
    {h_t} =  z_t \cdot h_{t-1} + (1-z_t)\cdot \widetilde{h_t}.
\end{equation}


\subsection{Forecasting model evaluation metric}
There are many metrics used in various studies to evaluate the forecasting model ability, and there is no uniform criterion for selecting evaluation metrics. In this work, three performance metric based on root mean squared error (RMSE), mean absolute error (MAE), and mean absolute percentage error (MAPE) are used to evaluate the model accuracy.
RMSE is a standard way to measure the error of prediction model. Let $x$ be the observed value, $\hat{x}$ is the predicted value, and $n$ is the number of observation.Then, RMSE can be defined as follows:
\begin{equation}\label{eq:RMSE}
    RMSE = \sqrt{\frac{1}{n}\sum_{i=1}^{n}{(x-\hat{x})}^2}.
\end{equation}
MAE measures the average magnitude of errors between predicted and observed value, which is mathematically indicated as follows:
\begin{equation}\label{eq:MAE}
    MAE = {\frac{1}{n}\sum_{i=1}^{n}{|x-\hat{x}|}}.
\end{equation}
MAPE is the computed average of percentage errors by which forecasts of a model differ from actual values of the quantity being forecast.The formula for MAPE is:
\begin{equation}\label{eq:MPE}
    MAPE = {\frac{100\%}{n}\sum_{i=1}^{n}|\frac{x-\hat{x}}{x}}|.
\end{equation}

\subsection{Preprocessing of Dataset}
Wind data obtained from an area in China\cite{Dataset}. The dataset contains various weather, turbine, and rotor features. Data has been recorded for an observation of every 10 minutes from January 2018 till March 2020. Initially, the dataset is preprocessed to visualize the relationship among dataset features. A data visualization based on correlation has been demonstrated in the form of a heat map in Fig. \ref{Heat}. 


%%%%%%%%%%%%%%%%% Edit %%%%%%%%%%%%%%%%%%%%%%%%%
The quality of data affects the performance of the machine learning model. So, it is necessary to clean and prepare data before processing it. Missing values in the dataset are imputed using mean values. After imputing missing values, data are transformed for processing. Data transformation is an essential pre-processing step that transforms data to the required scale or range. Standardization and normalization are various data transformation techniques. Standardization is a data preparation step where numerical values are converted to a common scale without degrading the results. The rescaled data will have a mean of 0 and a standard deviation of 1.



% \begin{figure}[h]
%   \centering
%     \includegraphics[scale=0.25, trim = 0.3cm 0.5cm 0.25cm 0.25cm, clip]{LSTM/Figures/Heatmap.png}
%     \caption{Heat map for data visualization}
%     \label{Heat}
%     % \vspace{-.2in}
% \end{figure}

\subsection{Forecasting results}
It can be seen that wind speed is the most correlated feature to the active power. In this work, we include wind speed, wind direction, temperature, and active power from the past 24 hours to develop a short term forecasting of wind power. First, the dataset has been restructured into a time-series format. Then, the data is divided into eighty percent (80\%) for training and twenty percent (20\%) for testing purpose of forecasting method. In order to make the dataset well-structured, the technique, which gives the structured or normalized values within the range of 0 and 1.
A stacked LSTM model consists of 64 neurons with linear activation function (Relu), the optimizer set to be Adam with learning rate of 0.001, the batch size is 64, and the number of iteration epochs is 20. To illustrate the efficiency of LSTM model in this case, three different methods also has been implemented and the table. \ref{table:Error} shows the comparison for these models.  Fig.\ref{Forecast} shows the forecasting result for next 24 hours.

\begin{figure}[h]
   \centering
    \includegraphics[scale=0.24, trim = 0.2cm 0.2cm 0.1cm 0.2cm, clip]{Figures/LSTM_Predict.png}
    \caption{LSTM predication for three different time horizon}
    \label{Barplot}
    % \vspace{-.2in}
\end{figure}



\begin{figure}[h]
   \centering
    \includegraphics[scale=0.4, trim = 0.1cm 0.1cm 0.1cm 0.1cm, clip]{Figures/models.png}
    \caption{Comparing various forecasting models for 3 hours time horizon prediction}
    \label{Forecast}
    % \vspace{-.2in}
\end{figure}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\caption{Error evaluation results for different models} 
\begin{tabular}{cllll}
\hline
\multicolumn{1}{l}{Ahead time (h)} & Model & RMSE    & MAE    & MAPE   \\ \hline
\multirow{3}{*}{1}                 & RNN   & 8.569 & 7.186 & 17.61\%  \\ \cline{2-5} 
                                   & LSTM  & 6.237      & 5.842    & 9.848\%      \\ \cline{2-5} 
                                   & GRU   & 6.857       & 6.152   & 16.25\%      \\ \hline
\multirow{3}{*}{12}                 & RNN   & 10.462 & 9.582 & 39.14\% \\ \cline{2-5} 
                                   & LSTM  & 8.521 & 7.024 & 34.148\%  \\ \cline{2-5} 
                                   & GRU   & 9.378       & 8.234      & 36.45\%      \\ \hline
\multirow{3}{*}{24}                 & RNN   & 11.873      & 10.479      & 44.58\%      \\ \cline{2-5} 
                                   & LSTM  & 9.287       & 7.862      & 38.573\%      \\ \cline{2-5} 
                                   & GRU   & 9.732       & 8.612      & 40.22\%      \\ \hline
\end{tabular}
\end{table}



% \begin{table}[ht]

% \centering 
% \caption{Error evaluation results for different models} 
% \begin{tabular}{c | c c c} 
% \hline\hline
% Model & RMSE    & MAE    & MAPE  \\  [0.5ex]
% \hline % inserts single horizontal line
% CNN   & 192.077 & 11.389 & 1.244 \\ % inserting body of the table
% RNN   & 151.053 & 9.85 & 1.243 \\
% LSTM  & 150.619 & 9.843 & 0.902 \\
% GRU   & 149.722 & 9.789 & 0.776 \\[1ex] % [1ex] adds vertical space
% \hline %inserts single line
% \end{tabular}
% \label{table:Error} % is used to refer this table in the text
% \end{table}




% The weight matrices are shown as $W_f$, $W_i$, and $W_o$ for forget, input and output gate respectively. The bias variables are also $b_f$, $b_i$, and $b_o$. 
